VL-SAT: Visual-Linguistic Semantics Assisted Training for 3D Semantic Scene Graph Prediction in Point Cloud

The task of 3D semantic scene graph (3DSSG) prediction in the point cloud is challenging since (1) the 3D point cloud only captures geometric structures with limited semantics compared to 2D images, and (2) long-tailed relation distribution inherently hinders the learning of unbiased prediction. Since 2D images provide rich semantics and scene graphs are in nature coped with languages, in this study, we propose Visual-Linguistic Semantics Assisted Training (VL-SAT) scheme that can significantly empower 3DSSG prediction models with discrimination about long-tailed and ambiguous semantic relations. The key idea is to train a powerful multi-modal oracle model to assist the 3D model. This oracle learns reliable structural representations based on semantics from vision, language, and 3D geometry, and its benefits can be heterogeneously passed to the 3D model during the training stage. By effectively utilizing visual-linguistic semantics in training, our VL-SAT can significantly boost common 3DSSG prediction models, such as SGFN and SGGpoint, only with 3D inputs in the inference stage, especially when dealing with tail relation triplets. Comprehensive evaluations and ablation studies on the 3DSSG dataset have validated the effectiveness of the proposed scheme. Code is available at https://github.com/wz7in/CVPR2023-VLSAT.

==> cvpr2023-cross-modal-3dssg/secs/exp.tex <==
% !TEX root = ../PaperForReview.tex

\begin{table*}
\centering
\caption{
%
Quantitative Results of 3D semantic scene graph prediction on the 3DSSG validation set~\cite{wald2020learning}. 
%
Evaluations are conducted in terms of object, predicate, and triplet. 
%
The results of SGPN, \sggpoint, and SGFN are based on our reproduced model with point cloud-only inputs, since they don't compute the mA@$k$ metric in their papers.
}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{Object} & \multicolumn{6}{c|}{Predicate} & \multicolumn{4}{c}{Triplet} \\
 \cline{2-14}
& A@$1$ & A@$5$ & A@$10$ & A@$1$ & A@$3$ & A@$5$ & mA@$1$ & mA@$3$ & mA@$5$ & A@$50$ & A@$100$ & mA@$50$ & mA@$100$ \\
 \hline
 SGPN~\cite{wald2020learning} & 48.28 & 72.94 & 82.74 & \textbf{91.32} & 98.09 & 99.15 & 32.01 & 55.22 & 69.44 & 87.55 & 90.66 & 41.52 & 51.92 \\
\sggpoint~\cite{zhang2021exploiting} & 51.42 & 74.56 & 84.15 & 92.4 & 97.78 & 98.92 & 27.95 & 49.98 & 63.15 & 87.89 & 90.16 & 45.02 & 56.03 \\
 SGFN~\cite{wu2021scenegraphfusion} & 53.67 & 77.18 & 85.14 & 90.19 & 98.17 & 99.33 & 41.89 & 70.82 & 81.44 & 89.02 & 91.71 & 58.37 & 67.61 \\
 \hline
%  \basetwo & \textbf{65.56} & \textbf{86.24} & \textbf{91.51} & 89.34 & 97.89 & 99.20 & 41.77 & 61.83 & 76.11 & \textbf{92.79} & \textbf{95.06} & 64.18 & \textbf{77.23} \\
 non-VL-SAT & 54.79 & 77.62 & 85.84 & 89.59 & 97.63 & 99.08 & 41.99 & 70.88 & 81.67 & 88.96 & 91.37 & 59.58 & 67.75 \\
%  \hline
%  Ours & 3D + 2D  & 65.88 & 86.53 & 91.46 & 90.78 & 55.66 & 98.45 & 78.61 & 99.56 & 89.82 & 93.09 & 74.10 & 95.22 & 81.38 \\
%  Ours & 3D + RGB & 51.87 & 76.35 & 84.19 & 91.28 & 48.52 & 98.49 & 70.45 & 99.42 & 78.10 & 88.74 & 56.76 & 91.46 & 65.67 \\
 VL-SAT (ours) & \textbf{55.66} & \textbf{78.66} & \textbf{85.91} & 89.81 & \textbf{98.45} & \textbf{99.53} & \textbf{54.03} & \textbf{77.67} & \textbf{87.65} & \textbf{90.35} & \textbf{92.89} & \textbf{65.09}  & \textbf{73.59} \\
 \hline
 VL-SAT (oracle) & 66.39 & 86.53 & 91.46 & 90.66 & 98.37 & 99.40 & 55.66 & 76.28 & 86.45 & 92.67 & 95.02 & 74.10 & 81.38 \\
 \hline
\end{tabular}}
\label{tab:exp-results}
\end{table*}

% \begin{table*}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c}
% \hline
% \multirow{2}{*}{Model} & \multicolumn{3}{c|}{Object} & \multicolumn{6}{c|}{Predicate} & \multicolumn{4}{c}{Triplet} \\
%  \cline{2-14}
%  & A@$1$ & A@$5$ & A@$10$ & A@$1$ & A@$3$ & A@$5$ & mA@$1$ & mA@$3$ & mA@$5$ & A@$50$ & A@$100$ & mA@$50$ & mA@$100$ \\
%  \hline
%  SGPN~\cite{wald2020learning} & 48.28 & 72.94 & 82.74 & \textbf{91.32} & 98.09 & 99.15 & 32.01 & 55.22 & 69.44 & 87.55 & 90.66 & 41.52 & 51.92 \\
% $\mathrm{\mathbf{SGG_{point}}}$~\cite{zhang2021exploiting} & 51.44 & 74.56 & 84.15 & 90.69 & 97.09 & 98.51 & 27.95 & 46.27 & 58.85 & 87.89 & 90.16 & 39.28 & 52.09 \\
%  SGFN~\cite{wu2021scenegraphfusion} & 53.67 & 77.18 & 85.14 & 90.19 & 98.17 & 99.33 & 41.89 & 70.82 & 81.44 & 89.02 & 91.71 & 58.37 & 67.61 \\
%  \hline
%  \basetwo & \textbf{65.56} & \textbf{86.24} & \textbf{91.51} & 89.34 & 97.89 & 99.20 & 41.77 & 61.83 & 76.11 & \textbf{92.79} & \textbf{95.06} & 64.18 & \textbf{77.23} \\
%  \basethree & 54.79 & 77.62 & 85.84 & 89.59 & 97.63 & 99.08 & 41.99 & 70.88 & 81.67 & 88.96 & 91.37 & 59.58 & 67.75 \\
%  \hline
% %  Ours & 3D + 2D  & 65.88 & 86.53 & 91.46 & 90.78 & 55.66 & 98.45 & 78.61 & 99.56 & 89.82 & 93.09 & 74.10 & 95.22 & 81.38 \\
% %  Ours & 3D + RGB & 51.87 & 76.35 & 84.19 & 91.28 & 48.52 & 98.49 & 70.45 & 99.42 & 78.10 & 88.74 & 56.76 & 91.46 & 65.67 \\
%  Ours & 55.66 & 78.66 & 85.91 & 89.81 & \textbf{98.45} & \textbf{99.53} & \textbf{54.03} & \textbf{77.67} & \textbf{87.65} & 90.35 & 92.89 & \textbf{65.09}  & 73.59 \\
%  \hline
% \end{tabular}}
% \caption{
% %
% 3D scene graph prediction performance on 3DSSG validation set. 
% %
% Evaluation is conducted in terms of object, predicate, and triplet. 
% %
% The results of SGPN, $\mathrm{\mathbf{SGG_{point}}}$, and SGFN are based on our reproduced model, since they don't compute the mA@$k$ metric in the paper.
% }
% \label{tab:exp-results-old}
% \end{table*}

\section{Experiments and Discussions}
\label{sec:experiments_and_discussions}

\subsection{Setups and Implementation Details}
\label{subsec:exp-setup}

\noindent\textbf{Datasets.} 
%
We conduct experiments on 3DSSG~\cite{wald2020learning}. It is a 3D semantic scene graph dataset drawn from the 3RScan dataset~\cite{wald2019rio}, with rich annotations about instance segmentation masks and relation triplets.
%
It has $1553$ 3D reconstructed indoor scenes, $160$ classes of objects, and $26$ types of predicates.
%
% We sample $128$ points from a segmented instances to represent a node entity. 
%
% As for relationship initialization, we use the relative location information of two objects.
%
In the experiments, we use the same data preparation and training/validation split as in 3DSSG~\cite{wald2020learning}.

\vspace{+1mm}
\noindent\textbf{Metrics and Tasks.} 
%
We follow the experiment settings in 3DSSG~\cite{wald2020learning} . 
%
In both training and testing stages, 3D scenes are placed in the same 3D coordinate. The view-dependent spatial relation predicates are not ambiguous.
% To evaluate our method comprehensively, we follow the scheme in \cite{wald2020learning}, \eg we compute the top-k accuracy (A@$k$) to evaluate object and predicate prediction performance, which is referred to as R@$k$ in \cite{wald2020learning}.
% 
To evaluate the prediction of the object and predicate, we use the top-k accuracy (A@$k$) metric.
%
As for the triplets, we first multiply the subject, predicate, and object scores to get triplet scores, and then compute the top-k accuracy (A@$k$) as the evaluation metric.
% 
The triplet is considered correct only if the subject, predicate, and object are all correct\footnote{However, the metric top-k accuracy is written as the top-k recall or R@k in 3DSSG~\cite{wald2020learning} and SGFN~\cite{wu2021scenegraphfusion}.}.
%
% To alleviate the effects of long-tail distribution on test results, we also computed the average of the predicate and triplet accuracy on each predicate class as the mean top-k accuracy (mA@$k$) metric, which is a common practice in 2D scene graph prediction task \cite{tang2019learning}.
To fairly evaluate the performance of long-tailed predicate distribution, we also compute the average top-k accuracy of the predicate across all predicate classes, denoted as the mean top-k accuracy (mA@$k$).
%

% To compare with the method in Zhang~\etal~\cite{zhang2021knowledge}, 
%
We also conduct two 2D scene graph tasks proposed in \cite{xu2017scene} in the 3D scenario, as what Zhang~\etal~\cite{zhang2021knowledge} did, \ie,
%
(1) Scene Graph Classification (SGCls) that \textcolor{black}{evaluates} the triplet together.
%
(2) Predicate Classification (PredCls) that only \textcolor{black}{evaluates} the predicate \textcolor{black}{with the ground-truth labels of object entities.}
% given that the subject and object are correct.
%
Following Zhang~\etal~\cite{zhang2021knowledge}, we compute the recall at the top-k (R@$k$) triplets.
%
The triplet is considered correct when the subject, predicate, and object are all valid.
%
% As defined in ~\cite{lu2016visual}, the recall is the fraction of the correct top-k triplets against the ground truth.
%
Additionally, we also adopt mean recall (mR@$k$) to evaluate the performance on the unevenly sampled relations using a similar strategy as mA@$k$.

\vspace{+1mm}
% \noindent\textbf{Network Train and Inference Details.}
\noindent\textbf{Implementation Details.} 
%
Our network is end-to-end optimized using AdamW optimizer~\cite{DBLP:journals/corr/KingmaB14,DBLP:journals/corr/abs-1711-05101} with the batch size as $8$.
%
We train the network for $100$ epochs, and the base learning rate is set as $0.001$ with a cosine annealing learning rate decay strategy~\cite{loshchilov2016sgdr}.
%
$N_\text{obj}=160$ and $N_\text{rel}=26$ in our experiments.
%
GNN modules are repeated for $T=2$ times in both 3D and oracle multi-modal models.
%
$\lambda_{\text{obj}}=\lambda_{\text{aux}}=0.1$, $\lambda_{\text{pred}}=1$ in \cref{eq:loss_total}.
%
All experiments are carried out on the PyTorch platform equipped with one NVIDIA GeForce RTX 2080 Ti GPU card, and each experiment takes about $48$ hours until model convergence.
% What should be noted is that the 2D inputs are only used during the training stage.
Note that 2D inputs are only used during the training stage.
% 
During the inference stage, we follow the same strategy in  ~\cite{xu2017scene}, which selects the top@$1$ class of both object and predicate while giving an object instance index tuple. 
% %
% Then we multiply the object score, subject score and predicate score as the triplet score.
% %
% In the end, we sorted all triplet scores and select top@$k$ as our model's output.
% TODO 模型类型
%
Please refer to the supplementary for the details of the network structures.
%


\subsection{Comparison with the State-of-the-art Methods}
\label{subsec:exp-results}
%
We compare our method with a list of reference methods, \ie SGPN~\cite{wald2020learning}, \sggpoint~\cite{zhang2021exploiting}, SGFN~\cite{wu2021scenegraphfusion}, Co-Occurrence~\cite{zhang2021knowledge}, KERN~\cite{chen2019knowledge}, Schemata~\cite{sharifzadeh2021classification}, Zhang~\etal~\cite{zhang2021knowledge}. 
%
% SGPN~\cite{wald2020learning} is the pioneer in 3D scene graph prediction tasks, which uses a simple PointNet~\cite{qi2017pointnet} with GNN to generate scene graph predictions.
% %
% The following work SGFN~\cite{wu2021scenegraphfusion} leverages an attention-based node feature updating strategy in GNN and incrementally builds up scene graphs from RGB-D sequences.
% %
% In this comparison, the online updating strategy of SGFN is blocked.
% %
% Zhang~\etal~\cite{zhang2021knowledge} uses a graph auto-encoder to automatically extract class-wise representations as prior knowledge to enhance relationship prediction.
% %
% $\text{SGG}_\text{point}$~\cite{zhang2021exploiting} builds two associated twin interaction mechanisms between nodes and edges to effectively bridge perception and reasoning.
%
In addition, to gain a deeper understanding of our approach, we also report the performances of the oracle multi-modal prediction model (termed as VL-SAT (oracle)), as well as the baseline performance of the 3D prediction model that is trained purely by 3D data (term as non-VL-SAT). The proposed method is term as VL-SAT.

% we design some variants of our method. \basetwo uses a similar network structure as the teacher network except for multi-level feature enhancements and takes in 2D image patches of objects and 3D bounding box positions in the train and validation process. \basethree adopts the same network as the student network and takes in 3D point clouds in both train and validation 
% period.

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{picture/freq.pdf}
\caption{
%
The line chart shows the predicate frequency in the train set of 3DSSG~\cite{wald2020learning}.
%
The bar chart shows the results on mA@$1$ of the predicate prediction of SGPN~\cite{wald2020learning} and our VL-SAT.
}
\label{fig:predicate_dis}
\end{figure}

\vspace{+1mm}
\noindent\textbf{Quantitative Results.}
%
The comparison results are summarized in \cref{tab:exp-results}.
%
The baseline ``non-VL-SAT'' has a similar performance as SGFN.
%
\textcolor{black}{The only difference between them is that ``non-VL-SAT'' adds a multi-head self-attention (MHSA) module~\cite{vaswani2017attention} before each GNN module in SGFN.}
%
Thanks to the delicate visual-linguistic assisted training scheme, our ``VL-SAT'' tremendously improves the baseline, according to the evaluation with respect to the predicate, and the triplet.
%
Moreover, according to the less biased mA@k metrics with respect to long-tailed distribution, when evaluating the predicate, the proposed ``VL-SAT'' outperforms the baseline ``non-VL-SAT'' with around $12.0\%$, $6.8\%$ and $6.0\%$ gains at mA@$1$, mA@$3$, and mA@$5$ respectively.
%
Our method reaches new state-of-the-art results on triplet prediction, with $6.8\%$ gain on mA@50 and $5.9\%$ gain on mA@100 over SGFN~\cite{wu2021scenegraphfusion}.
%
Note that the results of object classification just have a marginal improvement, which means that a simple PointNet-based 3D encoder may not be able to convey similar instance-level representative power as the 2D vision encoder.
%
% (TODO) It is interesting to find that our oracle model ``VL-SAT (oracle)'' further boosts the overall performance, but its gains mainly come from a better object classifier rather than better modeling of the predicate.

% Due to sufficient object texture and color information in 2D images, \basetwo performs well on object classification and brings about $12\%$ gains on A@$1$ compared with SGFN.
% %
% The shortcoming of \basetwo is also obvious. 
% %
% Because of lacking spatial information, \basetwo performs poorly on predicate prediction.
% %
% Our method gains $2\%$ improvement on object A@$1$ metric over SGFN~\cite{wu2021scenegraphfusion}, benefiting from the multi-level enhancement strategy.
% %
% As for the evaluation of predicate prediction, SGFN, \basethree, and our method all achieve remarkable performance on A@$k$ metric.
% %
% Regarding the mA@$k$ metric, which is less influenced by the long-tail distribution effect, our method outperforms SGFN by $12.2\%$ on the predicate mA@1 metric.
% %
% Thanks to the strong performance on the object and predicate prediction, our method reaches a new state-of-the-art result on triplet prediction, with $6.8\%$ gain on mA@50 and $5.9\%$ gain on mA@100 over SGFN\cite{wu2021scenegraphfusion}.


As illustrated in \cref{tab:exp-buaa1} and \cref{tab:exp-buaa2}, we also compare our ``VL-SAT'' with the reference methods, with respect to two tasks named SGCls and PredCls, according to the settings introduced by Zhang~\etal~\cite{zhang2021knowledge}.
%
Our method outperforms Zhang~\etal~\cite{zhang2021knowledge} by a large margin.
%
For example, with graph constraint~\cite{xu2017scene} (as a more rigorous testing scenario~\cite{zareian2020bridging}), ``VL-SAT'' has $2.5\%$ gain on R@$20$ in SGCls, $8.5\%$ gain on R@$20$ in PredCls.
%
Moreover, with respect to the less biased metrics in \cref{tab:exp-buaa2}, ``VL-SAT'' even achieves $6.6\%$ gains on mR@$20$ in SGCls than Zhang~\etal~\cite{zhang2021knowledge}.

% \begin{table*}
% \centering
% \resizebox{\linewidth}{!}{
%         \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c}
%         \hline
% \multirow{2}{*}{Model} & \multicolumn{3}{c|}{Object} & \multicolumn{6}{c|}{Predicate} & \multicolumn{4}{c}{Triplet} \\
%  \cline{2-14}
%  & R@$1$ & R@$5$ & R@$10$ & R@$1$ & mR@$1$ & R@$3$ & mR@$3$ & R@$5$ & mR@$5$ & R@$50$ & mR@$50$ & R@$100$ & mR@$100$ \\
%  \hline
%  SGPN~\cite{wald2020learning} & 48.28 & 72.94 & 82.74 & 91.32 & 32.01 & 98.09 & 55.22 & 99.15 & 69.44 & 87.55 & 41.52 & 90.66 & 51.92 \\
%  SGFN~\cite{wu2021scenegraphfusion} & 53.67 & 77.18 & 85.14 & 90.19 & 41.89 & 98.17 & 70.82 & 99.33 & 81.44 & 89.02 & 58.37 & 91.71 & 67.61 \\
%  \hline
%  $\mathrm{Base_{2d}}$ & \textbf{65.56} & \textbf{86.24} & \textbf{91.51} & 89.34 & 41.77 & 97.89 & 61.83 & 99.20 & 76.11 & \textbf{92.79} & 64.18 & \textbf{95.06} & \textbf{77.23} \\
%  \revise{$\mathrm{Base_{3d}}$} & 55.43 & 79.09 & 86.51 & \textbf{91.81} & 52.30 & \textbf{98.70} & 71.48 & \textbf{99.64} & 82.75 & 89.71 & 60.74 & 92.96 & 71.56 \\
%  \hline
% %  Ours & 3D + 2D  & 65.88 & 86.53 & 91.46 & 90.78 & 55.66 & 98.45 & 78.61 & 99.56 & 89.82 & 93.09 & 74.10 & 95.22 & 81.38 \\
% %  Ours & 3D + RGB & 51.87 & 76.35 & 84.19 & 91.28 & 48.52 & 98.49 & 70.45 & 99.42 & 78.10 & 88.74 & 56.76 & 91.46 & 65.67 \\
%  Ours & 55.66 & 78.66 & 85.91 & 89.81 & \textbf{54.03} & 98.45 & \textbf{77.67} & 99.53 & \textbf{87.65} & 90.35 & \textbf{65.09} & 92.89  & 73.59 \\
%  \hline
% \end{tabular}}
% \caption{
% %
% 3D scene graph prediction performance on 3DSSG validation set. 
% %
% Evaluation is conducted in terms of object, predicate, and triplet. 
% %
% The results of SGFN and SGPN are based on our reproduced model.
% %
% }
% \label{tab:exp-results}
% \end{table*}

\begin{table}
\caption{
%
Quantitative results of the compared methods with respect to the SGCls and PredCls tasks, with and without graph constraint. The evaluation metric is top-$k$ recall.
}
\label{tab:exp-buaa1}
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c}
\hline
\multicolumn{1}{c|}{}& SGCls & PredCls \\
\cline{2-3}
Model & R@$20$/$50$/$100$ & R@$20$/$50$/$100$ \\
\midrule
\multicolumn{3}{c}{with Graph Constraints} \\
\hline
Co-Occurrence~\cite{zhang2021knowledge} & 14.8/19.7/19.9 & 34.7/47.4/47.9 \\
KERN~\cite{chen2019knowledge} & 20.3/22.4/22.7 & 46.8/55.7/56.5 \\
SGPN~\cite{wald2020learning} & 27.0/28.8/29.0 & 51.9/58.0/58.5 \\
Schemata~\cite{sharifzadeh2021classification} & 27.4/29.2/29.4 & 48.7/58.2/59.1 \\
Zhang~\etal~\cite{zhang2021knowledge} & 28.5/30.0/30.1 & 59.3/65.0/65.3 \\
SGFN~\cite{wu2021scenegraphfusion} & 29.5/31.2/31.2 & 65.9/78.8/79.6 \\
VL-SAT (ours) & \textbf{32.0}/\textbf{33.5}/\textbf{33.7} & \textbf{67.8}/\textbf{79.9}/\textbf{80.8} \\
\midrule
\multicolumn{3}{c}{without Graph Constraints} \\
\hline
Co-Occurrence~\cite{zhang2021knowledge} & 14.1/20.2/25.8 & 35.1/55.6/70.6 \\
KERN~\cite{chen2019knowledge} & 20.8/24.7/27.6 & 48.3/64.8/77.2 \\
SGPN~\cite{wald2020learning} & 28.2/32.6/35.3 & 54.5/70.1/82.4 \\
Schemata~\cite{sharifzadeh2021classification} & 28.8/33.5/36.3 & 49.6/67.1/80.2 \\
Zhang~\etal~\cite{zhang2021knowledge} & 29.8/34.3/37.0 & 62.2/78.4/88.3 \\
SGFN~\cite{wu2021scenegraphfusion} & 31.9/39.3/45.0 & 68.9/82.8/91.2 \\
VL-SAT (ours) & \textbf{33.8}/\textbf{41.3}/\textbf{47.0} & \textbf{70.5}/\textbf{85.0}/\textbf{92.5} \\
\hline
\end{tabular}}
\end{table}

% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{cc|c|c|c|c|c|c}
% \hline
% \multicolumn{2}{c|}{}&\multicolumn{3}{|c|}{SGCls} & \multicolumn{3}{|c}{PredCls} \\
% \cline{3-8}
% & Model & R@$20$ & R@$50$ & R@$100$ & R@$20$ & R@$50$ & R@$100$ \\
% \hline
% \multirow{7}{*}{w/ GC} & Co-Occurrence~\cite{zhang2021knowledge} & 14.8 & 19.7 & 19.9 & 34.7 & 47.4 & 47.9 \\
% & KERN~\cite{chen2019knowledge} & 20.3 & 22.4 & 22.7 & 46.8 & 55.7 & 56.5 \\
% & SGPN~\cite{wald2020learning} & 27.0 & 28.8 & 29.0 & 51.9 & 58.0 & 58.5 \\
% & Schemata~\cite{sharifzadeh2021classification} & 27.4 & 29.2 & 29.4 & 48.7 & 58.2 & 59.1 \\
% & Zhang2021~\cite{zhang2021knowledge} & 28.5 & 30.0 & 30.1 & 59.3 & 65.0 & 65.3 \\
% & SGFN~\cite{wu2021scenegraphfusion} & 29.5 & 31.2 & 31.2 & 65.9 & 78.8 & 79.6 \\
% & Ours & \textbf{32.0} & \textbf{33.5} & \textbf{33.7} & \textbf{67.8} & \textbf{79.9} & \textbf{80.8} \\
% \hline 
% \multirow{7}{*}{w/o GC} & Co-Occurrence~\cite{zhang2021knowledge} & 14.1 & 20.2 & 25.8 & 35.1 & 55.6 & 70.6 \\
% & KERN~\cite{chen2019knowledge} & 20.8 & 24.7 & 27.6 & 48.3 & 64.8 & 77.2 \\
% & SGPN~\cite{wald2020learning} & 28.2 & 32.6 & 35.3 & 54.5 & 70.1 & 82.4 \\
% & Schemata~\cite{sharifzadeh2021classification} & 28.8 & 33.5 & 36.3 & 49.6 & 67.1 & 80.2 \\
% & Zhang2021~\cite{zhang2021knowledge} & 29.8 & 34.3 & 37.0 & 62.2 & 78.4 & 88.3 \\
% & SGFN~\cite{wu2021scenegraphfusion} & 31.9 & 39.3 & 45.0 & 68.9 & 82.8 & 91.2 \\
% & Ours & \textbf{33.8} & \textbf{41.3} & \textbf{47.0} & \textbf{70.5} & \textbf{85.0} & \textbf{92.5} \\
% \hline
% \end{tabular}}
% \caption{
% %
% Quantitative results of the evaluated methods in SGCls and PredCls tasks in recall, with and without graph constraint (GC).
% }
% \label{tab:exp-buaa1}
% \end{table}

\begin{table}
\centering
\caption{
%
Quantitative results of the compared methods with respect to the SGCls and PredCls tasks, with graph constraint. The evaluation metric is top-$k$ mean recall.
}
\label{tab:exp-buaa2}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{c|c|c}
\hline
&\multicolumn{1}{|c|}{SGCls} & \multicolumn{1}{|c}{PredCls} \\
\cline{2-3}
Model & mR@$20$/$50$/$100$ & mR@$20$/$50$/$100$ \\
\hline
Co-Occurrence~\cite{zhang2021knowledge} & 8.8/12.7/12.9 & 33.8/47.4/47.9 \\
KERN~\cite{chen2019knowledge} & 9.5/11.5/11.9 & 18.8/25.6/26.5 \\
SGPN~\cite{wald2020learning} & 19.7/22.6/23.1 & 32.1/38.4/38.9 \\
Schemata~\cite{sharifzadeh2021classification} & 23.8/27.0/27.2 & 35.2/42.6/43.3 \\
Zhang~\etal~\cite{zhang2021knowledge} & 24.4/28.6/28.8 & 56.6/63.5/63.8 \\
SGFN~\cite{wu2021scenegraphfusion} & 20.5/23.1/23.1 & 46.1/54.8/55.1 \\
VL-SAT(ours) & \textbf{31.0}/\textbf{32.6}/\textbf{32.7} & \textbf{57.8}/\textbf{64.2}/\textbf{64.3} \\
\hline 
\end{tabular}}
\end{table}

\begin{figure*}
\centering
\includegraphics[width=0.99\linewidth]{picture/3dssg.pdf}
\caption{
%
Qualitative results from SGFN~\cite{wu2021scenegraphfusion} and our method on the 3DSSG~\cite{wald2020learning} dataset.
%
\textit{Red edge}: miss-classified edges from SGFN, \textit{green edge}: edges corrected by our method, \textit{red node}: miss-classified node.
}
\label{fig:qualitative}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[width=0.95\linewidth]{picture/scannet.pdf}
\caption{
%
Qualitative results from SGFN~\cite{wu2021scenegraphfusion} and our method on ScanNet~\cite{dai2017scannet} dataset. 
%
Note that there are no annotations of scene graphs on ScanNet~\cite{dai2017scannet}, so we utilize the descriptions from ScanRefer~\cite{chen2020scanrefer} to parse the relationships between different objects manually.
%
\textit{Red edge}: miss-classified edges from SGFN, \textit{green edge}: edges corrected by our method, \textit{red node}: miss-classified node.
}
\label{fig:qualitative_scannet}
\end{figure*}

%
\begin{table*}
\centering
\caption{
%
Based on the distribution of the predicates in the train set of the 3DSSG dataset~\cite{wald2020learning}, we split the $26$ predicate classes into the head, body, and tail classes, and then compute mA@3 and mA@5 metrics on each split.
%
% Besides, we also split the predicate classes into spatial predicate and semantic predicate, based on whether the predicate describes a spatial relation.
%
Moreover, we test several methods on unseen and seen triplets in the validation set to evaluate the generalization ability of these methods.
}
\label{tab:long-tail}
\resizebox{0.8\linewidth}{!}{
        \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
\hline
\multirow{3}{*}{Model}& \multicolumn{6}{|c|}{Predicate} & \multicolumn{4}{|c}{Triplet} \\
\cline{2-11}
&\multicolumn{2}{c|}{Head} & \multicolumn{2}{|c|}{Body} & \multicolumn{2}{|c}{Tail} & \multicolumn{2}{|c|}{Unseen} & \multicolumn{2}{|c}{Seen} \\
 \cline{2-11}
& mA@$3$ & mA@$5$ &mA@$3$ & mA@$5$ & mA@$3$ & mA@$5$ & A@50 & A@100 & A@50 & A@100 \\
 \hline
 SGPN~\cite{wald2020learning} & \textbf{96.66} & 99.17 & 66.19 & 85.73 & 10.18 & 28.41 & 15.78 & 29.60 & 66.60 & 77.03  \\
 SGFN~\cite{wu2021scenegraphfusion} & 95.08 & \textbf{99.38} & 70.02 & 87.81 & 38.67 & 58.21 & 22.59 & 35.68 & 71.44 & 80.11 \\
 \hline
 non-VL-SAT & 95.32 & 99.01 & 71.88 & 88.64 & 40.01 & 58.33 & 21.99 & 35.44 & 71.52 & 80.34  \\
 VL-SAT (ours) & 96.31 & 99.21 & \textbf{80.03} & \textbf{93.64}  & \textbf{52.38} & \textbf{66.13} & \textbf{31.28} & \textbf{47.26} & \textbf{75.09} & \textbf{82.25} \\
 \hline
\end{tabular}}
\end{table*}

\vspace{+1mm}
\noindent\textbf{Qualitative Results.}
%
We provide some qualitative results between SGFN and our ``VL-SAT'' in \cref{fig:qualitative}.
%
These results demonstrate that our method can predict more reliable scene graphs with more accurate edges and nodes.
%
For example, our method successfully distinguishes some similar predicate, like \textit{standing on} versus \textit{supported by} and further disambiguates related instances, such as \textit{shower curtain} versus \textit{bath cabinet}.
%
The results conducted on ScanNet~\cite{dai2017scannet} in \cref{fig:qualitative_scannet} validate that VL-SAT is generalizable to more datasets.

\subsection{More Evaluations about Predicate and Triplet}
\label{subsec:exp-long-tail}

\noindent\textbf{Tail Predicates.} 
%
In \cref{fig:predicate_dis}, we visualize the frequency of the predicates in the train set as the line chart, which shows the long-tail distribution.
%
We also show the per-class predicate prediction performances of ``VL-SAT'' and SGFN~\cite{wald2020learning} in the bar chart.
%
Compared with SGFN, our method gets a significant improvement in the tail categories.
%
To further explore the improvements brought by ``VL-SAT'', we split the $26$ predicate classes into three parts: \textit{head}, \textit{body}, and \textit{tail} according to their frequencies in the train set, and calculate mA@$k$ metric.
%
In \cref{tab:long-tail}, we obtain $13.71\%$ improvement on mA@$3$ when predicting the predicate on tail categories.
%
\textcolor{black}{Compared with SGFN, our method slightly drops on some head classes but significantly increases on tail classes.
%
Since our VL-SAT boosts the overall performance by a large margin, such a slight performance degradation in head predicates is acceptable.}
%
We also provide some examples of tail predicates in \cref{fig:qualitative}.
%
In the top row, our method correctly predicts tail predicates like \textit{supported by}.
%
In the bottom row, our method corrects the relation between the kitchen counter and the kitchen cabinet from \textit{attached to} to \textit{part of}.

% Definition of tail predicates can be found in supplementary.

% \noindent\textbf{Semantic predicate analysis.}
% %
% \revise{To show the gains on the predicate which contains semantic information, we also split the $26$ predicates into two parts, \eg predicates about the spatial structure like behind, and the semantic predicates like same as.
% %
% In table \ref{tab:long-tail}, we also obtain about $12\%$ and $7\%$ improvements on mR@$3$ and mR@$5$ of predicate evaluation on the semantic predicates, respectively.
% %
% The above result convinces us that, our methods not only ease the long-tail distribution on the training dataset but also introduce the semantic information on the spatial-only input.}

\vspace{+1mm}
\noindent\textbf{Unseen Triplets.} 
%
We consider relation triplets that do not appear in the train set as unseen triplets. 
%
In \cref{tab:long-tail}, our method gains about $8.69\%$ on A@$50$ on unseen triplets compared with SGFN~\cite{wald2020learning}.
%
The results validate that thanks to the VL-SAT scheme, our model can convey more robust feature representations based on the 3D point cloud, which leads to a better generalization ability on unseen triplets.


%
% The results show that our method performs well on tail predicates.

% \begin{table*}
% \centering
% \resizebox{\linewidth}{!}{
%         \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
% \hline
% \multirow{3}{*}{Model}& \multicolumn{6}{|c|}{Predicate} & \multicolumn{4}{|c|}{Predicate} & \multicolumn{4}{|c}{Triplet} \\
% \cline{2-15}
% &\multicolumn{2}{c|}{Head} & \multicolumn{2}{|c|}{Body} & \multicolumn{2}{|c}{Tail} & \multicolumn{2}{|c}{Spatial} & \multicolumn{2}{|c}{Semantic} & \multicolumn{2}{|c|}{Unseen} & \multicolumn{2}{|c}{Seen} \\
%  \cline{2-15}
% & mA@$3$ & mA@$5$ &mA@$3$ & mA@$5$ & mA@$3$ & mA@$5$  & mA@$3$ & mA@$5$ & mA@$3$ & mA@$5$ & A@50 & A@100 & A@50 & A@100 \\
%  \hline
%  SGPN & \textbf{96.66} & 99.17 & 66.19 & 85.73 & 10.18 & 28.41 & \textbf{82.76} & 85.97 & 39.53 & 57.22 & 15.78 & 29.60 & 66.60 & 77.03  \\
%  SGFN & 95.08 & \textbf{99.38} & 70.02 & 87.81 & 38.67 & 58.21 & 81.98 & \textbf{86.87} & 58.07 & 75.89 & 22.59 & 35.68 & 71.44 & 80.11 \\
%  \hline
%  \basethree & 95.32 & 99.01 & 71.88 & 88.64 & 40.01 & 58.33 & 81.41 & 86.17 & 60.19 & 75.33 & 21.99 & 35.44 & 71.52 & 80.34  \\
%  Ours & 96.31 & 99.21 & \textbf{80.03} & \textbf{93.64}  & \textbf{52.38} & \textbf{66.13} & 82.57 & 86.66 & \textbf{70.14} & \textbf{82.76} & \textbf{31.28} & \textbf{47.26} & \textbf{75.09} & \textbf{82.25} \\
%  \hline
% \end{tabular}}
% \caption{
% %
% Based on the frequency of the predicates in the train set, we split the $26$ classes of predicates into the head, body, and tail classes, and then compute mA@3 and mA@5 on each split.
% %
% Besides, we also split the predicate classes into spatial predicate and semantic predicate, based on whether the predicate describes a spatial relation.
% %
% Moreover, we test several methods on unseen and seen triplets in the validation set to evaluate the generalization ability of these methods.
% }
% \label{tab:long-tail}
% \end{table*}

\begin{table}
\centering
\caption{
%
Results of our method when different modules are ablated.
%
CI means CLIP-initialized object classifier.
% 
NC means node-level collaboration.
%
EC means edge-level collaboration.
%
TR means triplet-level CLIP-based regularization.
}
\label{tab:ablation_exp}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{CI} & \multirow{2}{*}{NC} & \multirow{2}{*}{EC} & \multirow{2}{*}{TR} & \multicolumn{2}{|c|}{Object} & \multicolumn{2}{|c|}{Predicate} & \multicolumn{2}{|c}{Triplet} \\
\cline{5-10}
& & & & A@$5$ & A@$10$ & mA@$3$ & mA@$5$ & mA@$50$ & mA@$100$ \\
\hline
% & & & & 77.62 & 85.84 & 70.88 & 81.67 & 59.58 & 67.75 \\
% \checkmark & & & & 79.03 & 86.81 & 72.50 & 83.59 & 60.65\color{red}{$\uparrow$1.07} & 69.71 \\
% \checkmark & \checkmark & & & \textbf{79.28} & \textbf{86.82} & 73.92 & 84.78 & 62.88\color{red}{$\uparrow$2.23} & 71.84 \\
% \checkmark & \checkmark & \checkmark & & 78.71 & 86.17 & 76.92 & 87.08 & 64.00\color{red}{$\uparrow$1.12} & 72.42 \\
% \checkmark & \checkmark & \checkmark & \checkmark & 78.66 & 85.91  & \textbf{77.67} & \textbf{87.65} & \textbf{65.09}\color{red}{$\uparrow$1.09} & \textbf{73.59} \\
& & & & 77.62 & 85.84 & 70.88 & 81.67 & 59.58 & 67.75 \\
\checkmark & & & & 79.03 & 86.81 & 72.50 & 83.59 & 60.65 & 69.71 \\
\checkmark & \checkmark & & & \textbf{79.28} & \textbf{86.82} & 73.92 & 84.78 & 62.88 & 71.84 \\
\checkmark & \checkmark & \checkmark & & 78.71 & 86.17 & 76.92 & 87.08 & 64.00 & 72.42 \\
\checkmark & \checkmark & \checkmark & \checkmark & 78.66 & 85.91  & \textbf{77.67} & \textbf{87.65} & \textbf{65.09} & \textbf{73.59} \\
\hline
\end{tabular}}
\end{table}

% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
% \hline
% \multirow{2}{*}{CI} & \multirow{2}{*}{OE} & \multirow{2}{*}{RE} & \multirow{2}{*}{TE} & \multicolumn{3}{|c|}{Object} & \multicolumn{3}{|c|}{Predicate} & \multicolumn{2}{|c}{Triplet} \\
% \cline{5-12}
% & & & & A@$1$ & A@$5$ & A@$10$ & mA@$1$ & mA@$3$ & mA@$5$ & mA@$50$ & mA@$100$ \\
% \hline
% & & & & 54.79 & 77.62 & 85.84 & 41.99 & 70.88 & 81.67 & 59.58 & 67.75 \\
% \checkmark & & & & 56.31 & 79.03 & 86.81 & 52.01\color{red}{$\uparrow$10.02} & 72.50\color{red}{$\uparrow$1.62} & 83.59 & 60.65\color{red}{$\uparrow$1.07} & 69.71 \\
% \checkmark & \checkmark & & & 55.89 & \textbf{79.28} & \textbf{86.82} & 52.52\color{red}{$\uparrow$0.51} & 73.92\color{red}{$\uparrow$1.42} & 84.78 & 62.88\color{red}{$\uparrow$2.23} & 71.84 \\
% \checkmark & \checkmark & \checkmark & & \textbf{56.40} & 78.71 & 86.17 & 53.55\color{red}{$\uparrow$1.03} & 76.92\color{red}{$\uparrow$3.00} & 87.08 & 64.00\color{red}{$\uparrow$1.12} & 72.42 \\
% \checkmark & \checkmark & \checkmark & \checkmark & 55.66 & 78.66 & 85.91 & \textbf{54.03}\color{red}{$\uparrow$0.48} & \textbf{77.67}\color{red}{$\uparrow$0.75} & \textbf{87.65} & \textbf{65.09}\color{red}{$\uparrow$1.09} & \textbf{73.59} \\
% \hline
% \end{tabular}}
% \caption{
% %
% Results of our method when different modules are ablated.
% %
% CI means CLIP-initialized object classifier.
% % 
% OE means object-level feature enhancement.
% %
% RE means relation-level feature enhancement.
% %
% TE means triplet-level feature enhancement.
% }
% \label{tab:ablation_exp_old}
% \end{table}

% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
% \hline
% \multirow{2}{*}{CI} & \multirow{2}{*}{OE} & \multirow{2}{*}{RE} & \multirow{2}{*}{TE} & \multicolumn{3}{|c|}{Object} & \multicolumn{3}{|c|}{Predicate} & \multicolumn{2}{|c}{Triplet} \\
% \cline{5-12}
% & & & & A@$1$ & A@$5$ & A@$10$ & mA@$1$ & mA@$3$ & mA@$5$ & mA@$50$ & mA@$100$ \\
% \hline
% % & & & & 54.79 & 77.62 & 85.84 & 41.99 & 70.88 & 81.67 & 59.58 & 67.75 \\
% $\times$ & \checkmark & \checkmark & $\times$ & 55.53\color{green}{$\downarrow$0.13} & 78.36 & 86.24 & 49.51\color{green}{$\downarrow$4.52} & 73.70 & 85.12 & 63.56\color{green}{$\downarrow$1.53} & 72.10 \\
% $\times$ & \checkmark & \checkmark & \checkmark & - & - & - & - & - & - & - & - \\
% \checkmark & $\times$ & \checkmark & \checkmark & 55.28\color{green}{$\downarrow$0.38} & 78.9 & 86.41 & 50.04\color{green}{$\downarrow$3.99} & 71.59 & 81.37 & 61.56\color{green}{$\downarrow$3.53} & 71.05 \\
% \checkmark & \checkmark & $\times$ & \checkmark & 56.59\color{red}{$\uparrow$0.93} & 78.38 & 86.66 & 51.54\color{green}{$\downarrow$2.49} & 77.32 & 87.09 & 64.16\color{green}{$\downarrow$0.93} & 72.93 \\
% \checkmark & \checkmark & \checkmark & $\times$ & 56.40\color{red}{$\uparrow$0.74} & 78.71 & 86.71 & 53.55\color{green}{$\downarrow$0.48} & 76.92 & 87.08 & 64.00\color{green}{$\downarrow$1.09} & 72.42 \\
% \checkmark & \checkmark & \checkmark & \checkmark & 55.66 & 78.66 & 85.91 & 54.03 & 77.67 & 87.65 & 65.09 & 73.59 \\
% \hline
% \end{tabular}}
% \caption{
% %
% Results of our method when different modules are ablated.
% %
% CI means CLIP-initialized object classifier.
% % 
% OE means object-level feature enhancement.
% %
% RE means relation-level feature enhancement.
% %
% TE means triplet-level feature enhancement.
% }
% \label{tab:ablation_exp1}
% \end{table}

\begin{table}
\centering
\caption{
%
Our method with different cross-modal collaboration operations.
% 
NC means node-level collaboration.
%
EC means edge-level collaboration.
%
CT means concatenation.
%
% MC means mimic.
%
% KNN means k-nearest neighbor.
%
CA means cross-attention in our method.
}
\label{tab:fusion}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{NC} & \multirow{2}{*}{EC} & \multicolumn{2}{|c|}{Object} & \multicolumn{2}{|c|}{Predicate} & \multicolumn{2}{|c}{Triplet} \\
\cline{3-8}
& & A@$1$ & A@$5$ & mA@$1$ & mA@$3$ & mA@$50$ & mA@$100$ \\
\hline
% MC & MC & - & -& -& -& -& -& -& - \\
% MC & CA & - & -& -& -& -& -& -& - \\
% CA & MC & - & -& -& -& -& -& -& - \\
% \hline
% CT & CT & 55.78 & 77.58 & 85.23 & 51.64 & 74.13 & 83.49 & 60.37\color{green}{$\downarrow$4.72} & 72.66 \\
% CT & CA & 56.14 & 78.38 & 86.60 & 52.28 & 75.04 & 84.52 & 61.50\color{green}{$\downarrow$3.59} & 73.80 \\
% CA & CT & 56.00 & 77.68 & 85.86 & 52.14 & 73.54 & 87.55 & 63.92\color{green}{$\downarrow$1.17} & 73.10 \\
CT & CT & 55.78 & 77.58 & 51.64 & 74.13 & 60.37 & 72.66 \\
CT & CA & 56.14 & 78.38 & 52.28 & 75.04 & 61.50 & 73.80 \\
CA & CT & 56.00 & 77.68 & 52.14 & 73.54 & 63.92 & 73.10 \\
\hline
% KNN & KNN & - & -& -& -& -& -& -& - \\
% KNN & CA & 55.51 & 78.12 & 85.71 & 52.88\color{green}{$\downarrow$1.15} & 75.83 & 87.02 & 63.67\color{green}{$\downarrow$1.42} & 73.26 \\
% CA & KNN & 55.47 & 78.10 & 86.15 & 52.27\color{green}{$\downarrow$1.76} & 73.92 & 87.98 & 64.14\color{green}{$\downarrow$0.95} & 73.39 \\
% \hline
CA & CA & 55.66 & 78.66 & 54.03 & 77.67 & 65.09 & 73.59 \\
\hline
\end{tabular}}
\end{table}

% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
% \hline
% \multirow{2}{*}{OE} & \multirow{2}{*}{RE} & \multicolumn{3}{|c|}{Object} & \multicolumn{3}{|c|}{Predicate} & \multicolumn{2}{|c}{Triplet} \\
% \cline{3-10}
% & & A@$1$ & A@$5$ & A@$10$ & mA@$1$ & mA@$3$ & mA@$5$ & mA@$50$ & mA@$100$ \\
% \hline
% % MC & MC & - & -& -& -& -& -& -& - \\
% % MC & CA & - & -& -& -& -& -& -& - \\
% % CA & MC & - & -& -& -& -& -& -& - \\
% % \hline
% % CT & CT & - & -& -& -& -& -& -& - \\
% CT & CA & 56.14 & 78.38 & 86.60 & 52.28\color{green}{$\downarrow$1.75} & 75.04 & 84.52 & 61.50\color{green}{$\downarrow$3.59} & 73.80 \\
% CA & CT & 56.00 & 77.68 & 85.86 & 52.14\color{green}{$\downarrow$1.89} & 73.54 & 87.55 & 63.92\color{green}{$\downarrow$1.17} & 73.10 \\
% \hline
% % KNN & KNN & - & -& -& -& -& -& -& - \\
% % KNN & CA & 55.51 & 78.12 & 85.71 & 52.88\color{green}{$\downarrow$1.15} & 75.83 & 87.02 & 63.67\color{green}{$\downarrow$1.42} & 73.26 \\
% % CA & KNN & 55.47 & 78.10 & 86.15 & 52.27\color{green}{$\downarrow$1.76} & 73.92 & 87.98 & 64.14\color{green}{$\downarrow$0.95} & 73.39 \\
% % \hline
% CA & CA & 55.66 & 78.66 & 85.91 & 54.03 & 77.67 & 87.65 & 65.09 & 73.59 \\
% \hline
% \end{tabular}}
% \caption{
% %
% Our method with different cross-modal enhancement strategies.
% % 
% OE means object-level feature enhancement.
% %
% RE means relation-level feature enhancement.
% %
% CT means concatenation.
% %
% % MC means mimic.
% %
% % KNN means k-nearest neighbour.
% %
% CA means cross-attention in our method.
% }
% \label{tab:fusion}
% \end{table}

% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \hline
% \multirow{2}{*}{\#GNN} & \multicolumn{3}{|c|}{Object} & \multicolumn{3}{|c|}{Predicate} & \multicolumn{2}{|c}{Triplet} \\
% \cline{2-9}
% & A@$1$ & A@$5$ & A@$10$ & mA@$1$ & mA@$3$ & mA@$5$ & mA@$50$ & mA@$100$ \\
% \hline
% $1$ & \textbf{55.76} & 78.40 & \textbf{86.79} & 48.54 & 68.45 & 77.60 & 57.10 & 70.91 \\
% $2$ & 55.66 & \textbf{78.66} & 85.91 & \textbf{54.03} & \textbf{77.67} & \textbf{87.65} & \textbf{65.09} & \textbf{73.59} \\
% $3$ & 55.09 & 77.39 & 85.33 & 42.24 & 67.84 & 83.93 & 62.54 & 71.13 \\
% $4$ & 53.95 & 76.99 & 84.78 & 40.10 & 63.64 & 79.47 & 61.37 & 71.08 \\
% \hline
% \end{tabular}}
% \caption{
% Performance of our method when different number of GNN layers are used.
% }
% \label{tab:gnn}
% \end{table}

\begin{table}
\centering
\caption{
%
Performance gains brought by our VL-SAT scheme with two reference 3DSSG prediction models.
}
\label{tab:sgg}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c}
\hline
& \multicolumn{2}{|c|}{Object} & \multicolumn{2}{|c|}{Predicate} & \multicolumn{2}{|c}{Triplet} \\
\cline{2-7}
& A@$1$ & A@$5$ & mA@$1$ & mA@$3$ & mA@$50$ & mA@$100$ \\
\hline
\sggpoint~\cite{zhang2021exploiting} & 51.42 & 74.56 & 27.95 & 49.98 & 45.02 & 56.03 \\
+VL-SAT & 52.08 & 75.76 & 38.04 & 60.36 & 52.51 & 64.31 \\
\hline
%  non-VL-SAT & 54.79 & 77.62 & 41.99 & 70.88 & 59.58 & 67.75 \\
%  VL-SAT (ours) & 55.66 & 78.66 & 54.03 & 77.67 & 65.09 & 73.59 \\
SGFN~\cite{wu2021scenegraphfusion} & 53.67 & 77.18 & 41.89 & 70.82 & 58.37 & 67.61 \\
+VL-SAT & 55.43 & 78.88 & 52.91 & 72.37 & 63.57 & 72.02 \\
\hline
\end{tabular}}
\end{table}




\subsection{Ablation Study and Analysis}
\label{subsec:ablation}

\noindent\textbf{Ablation Study.} 
%
In \cref{tab:ablation_exp}, we conduct a comprehensive ablation study.
%
The first row denotes the baseline method ``no-VL-SAT''.
% 
From \cref{tab:ablation_exp}, we could observe that the
%
% CLIP-initialized object classifier brings about $1.41\%$ gains on object A@$5$ and $1.62\%$ gains on predicate mA@$3$.
%
CLIP-initialized object classifier brings about $1.41\%$ gains on object A@$5$.
%
Node and edge-level collaboration and triplet-level CLIP-based regularization steadily bring gains on triplet prediction, with $2.23\%$, $1.12\%$, and $1.09\%$ boost on mA@$50$ metric. 
%
% The ablation study well demonstrates the effectiveness of each designed component.
%
\textcolor{black}{It is worth noting that regularizing the training of predicates and triplets may bring bias to the representation of objects, which leads to a slight drop in object prediction when EC/TR is employed.
%
Thanks to the NC/CI modules, this degradation is not severe, which validates the effectiveness of our VL-SAT training scheme.}

\vspace{+1mm}
\noindent\textbf{Different Cross-modal Collaboration Strategies.} 
%
We investigate the effects of different cross-modal collaboration operations in~\cref{tab:fusion}.
%
We compare a simple operation named CT, in which we just concatenate corresponding features between two models.
%
% CT can be applied to either node or edge-level collaboration.
%
When CT is applied, the mA@$50$ metric of the triplet prediction drops significantly.
%
% By employing our multi-head cross-attention (termed as CA) in both collaborations, significant gains in predicate and triplet predication can be observed.
%
By employing our multi-head cross-attention (termed as CA) in both collaborations, significant gains can be observed.
%
% The results show the effectiveness of  modules used in node and edge-level collaboration.

% \vspace{+1mm}
% \noindent\textbf{Number of GNN layers.} 
% %
% With more GNN layers, the performance of our method first increases and then drops, and the watershed is $2$.
% %
% So, we choose to use $2$ layers of GNN in our method.

\vspace{+1mm}
\noindent\textbf{Generalization Ability.}
%
In \cref{tab:sgg}, we also show the performance gains brought by our VL-SAT scheme with two reference 3DSSG prediction models, namely \sggpoint~\cite{zhang2021exploiting} and SGFN~\cite{wu2021scenegraphfusion}.
%
VL-SAT shows consistent performance gains with different 3D prediction models, especially with respect to the evaluation of predicate and triplet.
%
% The results demonstrate the effectiveness of VL-SAT when a different model is adopted.
% The results demonstrate the VL-SAT scheme is generalizable to common 3DSSG prediction models.

==> cvpr2023-cross-modal-3dssg/secs/intro.tex <==
% !TEX root = ../PaperForReview.tex


\section{Introduction}
\label{sec:intro}

Structurally understanding 3D geometric scenes is particularly important for tasks that require interaction with real-world environments, such as AR/VR~\cite{qi2019deep,zhao2021transformer3d,cheng2021back,shi2020points,shi2019pointrcnn,shi2020pv,zhang2020h3dnet} and navigation~\cite{cai20223djcg,he2021transrefer3d,chen2020scanrefer}.
%
As one vital topic in this field, predicting 3D semantic scene graph (3DSSG) in point cloud~\cite{wald2020learning} has received emerging attention in recent years.
%
% Specifically, given the point cloud of a 3D scene that is associated with class-agnostic 3D instance masks, the 3DSSG prediction task would like to construct a directed graph whose nodes are semantic labels of the 3D instances and the edges recognize the directional semantic or geometrical relations (termed as \emph{predicate}) between connected 3D instances (termed as \emph{subject} and \emph{object}), respectively.
%
Specifically, given the point cloud of a 3D scene that is associated with class-agnostic 3D instance masks, the 3DSSG prediction task would like to construct a directed graph whose nodes are semantic labels of the 3D instances and the edges recognize the directional semantic or geometrical relations between connected 3D instances.

% Thus, each relation in the scene graph can be represented as a triplet $\langle \emph{subject}, \emph{predicate}, \emph{object} \rangle$.
%
% The core problem of this task is to explore how to associate the subject and object pairs and understand their relations, in the form of relation triplets $\langle \emph{subject}, \emph{predicate}, \emph{object} \rangle$.

% Unlike 2D semantic scene graph (2DSSG) prediction studies the semantics can be captured in images 

\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{picture/teaser.pdf}
\caption{
\textbf{Comparison between previous method and our VL-SAT.}
%
(a) SGPN~\cite{wald2020learning}, as the 3D model, fails to find capture predicates such as \emph{build in}.
%
(b) VL-SAT creates an oracle model by heterogeneously fusing 2D semantics, and language knowledge along with the geometrical features, and the 3D model receives benefits from the oracle model during training.
%
During inference, the enhanced 3D model can correctly detect the tail predicates.}
\label{fig:teaser}
\end{figure}


However, in addition to common difficulties faced by scene graph prediction, there are several challenges specified to the 3DSSG prediction task. (1) 3D data such as point clouds only capture the geometric structures of each instance and may superficially define the relations by relative orientations or distances.
%
(2) Recent 3DSSG predication datasets~\cite{wald2020learning,zhang2021exploiting} are quite small and suffer from long-tailed predicate distributions, where semantic predicates are often rarer than geometrical predicates.
%
For example, as shown in \cref{fig:teaser}, the pioneering work SGPN~\cite{wald2020learning} usually prefers a simple and common geometric predicate \emph{standing on} between \emph{sink} and \emph{bath cabinet}, while the ground-truth relation triplet $\langle \emph{sink}, \emph{build in}, \emph{bath cabinet}\rangle$ cares more about the semantics, and the frequency of \emph{build in} in the training dataset is quite low, as shown in \cref{fig:predicate_dis}(a).
%
Even though some attempts~\cite{zhang2021knowledge,wu2021scenegraphfusion,zhang2021exploiting} have been proposed thereafter, the inherent limitations of the point cloud data to some extent hinder the effectiveness of these methods.

%
Since 2D images provide rich and meaningful semantics, and the scene graph prediction task is in nature aligned with natural languages, we explore using visual-linguistic semantics to assist the training, as another pathway to essentially enhance the capability of common 3DSSG prediction models with the aforementioned challenges.

How to assist 3D structural understanding with visual-linguistic semantics remains an open problem.
%
Previous studies mainly focus on employing 2D semantics to enhance instance-level tasks, such as object detection~\cite{qi2018frustum,qi2020imvotenet,bai2022transfusion,sindagi2019mvx}, visual grounding and dense captioning~\cite{zhao20213dvg,cai20223djcg,chen2020scanrefer,yuan2022x}.
%
Most of them require visual data both in training and inference, but a few of them, such as SAT~\cite{yang2021sat} and $\cX$-Trans2Cap~\cite{yuan2022x} treat 2D semantics as auxiliary training signals and thus offer more practical inference only with 3D data.
%
But these methods are specified to instance-level tasks and require delicately designed networks for effective assistance, thus they are less desirable to our structural prediction problem. 
%
Thanks to the recent success of large-scale cross-modal pretraining like CLIP~\cite{radford2021learning}, 2D semantics in images can be well aligned with linguistic semantics in natural languages, and the visual-linguistic semantics have been applied for alleviating long-tailed issue in tasks related to 2D scene graphs~\cite{zareian2020bridging, abdelkarim2021exploring, tang2019learning, tang2020unbiased} and human-object interaction~\cite{liao2022gen}.
%
But how to adapt similar assistance of visual-linguistic semantics to the 3D scenario remains unclear.


In this study, we propose the Visual-Linguistic Semantics Assisted Training (VL-SAT) scheme to empower the point cloud-based 3DSSG prediction model (termed as the 3D model) with sufficient discrimination about long-tailed and ambiguous semantic relation triplets.
%
In this scheme, we simultaneously train a powerful multi-modal prediction model as the oracle (termed as oracle model) that is heterogeneously aligned with the 3D model, which captures reliable structural semantics by extra data from vision, extra training signals from language, as well as the geometrical features from the 3D model. These introduced visual-linguistic semantics have been aligned by CLIP.
%
Consequently, the benefits of the oracle model, especially the multi-modal structural semantics, can be efficiently embedded into the 3D model through the back-propagated gradient flows.
%
In the inference stage, the 3D model can perform superior 3DSSG prediction performance with only 3D inputs. For example, in \cref{fig:teaser}(b), the predicate \emph{build in} can be reliably detected.
%
To our best knowledge, VL-SAT is the first visual-linguistic knowledge transfer work that is applied to 3DSSG prediction in the point cloud.
%
Moreover, VL-SAT can successfully enhance  SGFN~\cite{wu2021scenegraphfusion} and $\text{SGG}_\text{point}$~\cite{zhang2021exploiting}, validating that this scheme is generalizable to common 3DSSG prediction models.


We benchmark VL-SAT on the 3DSSG dataset~\cite{wald2020learning}. Quantitative and qualitative evaluations, as well as comprehensive ablation studies, validate that the proposed training scheme leads to significant performance gains, especially for tail relations, as discussed in \cref{sec:experiments_and_discussions}.

% As one of the fundamental tasks that aim at understanding the 3D visual world, 3D Scene Graph Prediction ...
% % insert figure
% The contribution of our paper can be summarized as: (1) to our best knowledge, it is the first time ... (2) (3)
% %
% You can refer it in \href{https://docs.qq.com/doc/DTEZxSU95cGdVWmVi}{introduction}

% As one of the fundamental tasks that aim at understanding the visual world better, scene graph prediction[2d sgg refs] aims to build a common structural representation that encodes the semantic elements and the complex relationships between them.
% % 
% Recently, some works~\cite{wald2020learning} have tried to generate scene graphs directly from 3D point clouds to restore the spatial information lost in 2D images, which can benefit the VR/AR and robot navigation tasks more.
% % 
% Specifically, given point clouds of a scene along with the object segmentation mask, 3D scene graph prediction aims to predict the object semantic class along with the relationships between different objects.
%

%
% However, there are still some problems in 3D scene graph prediction tasks, which hinder the performance of existing methods.
% %
% 1) The lack of texture information in 3D point clouds restrains a better understanding of the scene, which leads to a spatial-only relation prediction.
%
% As shown in Figure~\ref{fig:teaser}, the model prefers to predict a spatial-related relationship \textit{standing on} between sink and cabinet, while the ground-truth relationship is \textit{build in}.
%
% Utilizing the 2D semantic information by projecting 3D objects to 2D images to enrich the point clouds is a common practice to alleviate the problem in other 3D tasks, like 3D detection~\cite{qi2018frustum,qi2020imvotenet,bai2022transfusion,sindagi2019mvx} and 3D Visual Grounding~\cite{zhao20213dvg,cai20223djcg,chen2020scanrefer}.
% %
% However, these methods require extra 2D inputs in both train and inference stages, which brings a computation burden.
% %
% SAT~\cite{yang2021sat} proposes a method with an attention mask to prevent the network from utilizing 2D knowledge directly during training, which alleviates performance dropping only using 3d during inference.
% %
% But it fuses the multi-modal tokens with a union transformer encoder with the object-level only knowledge enhancement, which has a great limitation on the relation inference with a larger computation burden.
% %
% Similarly, X-Trans2Cap~\cite{yuan2022x} utilizes a similar idea to assist 3D dense caption tasks only during training with two modality transformer encoders.
% %
% But it only focuses on the same instance between two modalities, which ignores the hard negative instances in the scene.
% %
% 2) 3D scene graph prediction task suffers from a relatively small dataset size and long-tail distribution of predicates, which makes it difficult to do well on some tail categories. 
% %
% As shown in Figure xxx, the data distribution is very uneven, and in some categories, the previous method cannot distinguish them at all.
% %
% Zhang2021~\cite{zhang2021knowledge} generates a meta embedding from the training dataset to ease the long-tail problem on 3DSSG, which can be seen as a re-balance method.
% %
% But it can not bring new extra knowledge essentially.
% %
% Recently, thanks to a large amount of 2D data, CLIP connects the two modalities, image, and text, to achieve a better representation extraction effect and solve the long-tail distribution problem to some extent. 
% %
% So we hope that we can assist 3D learning with this generic multi-modal representation information during training and expect to achieve better results.
%

% To address the above problems, we propose a multi-modal knowledge-assisted model while ensuring that the original 3D scene graph structure remains largely unchanged with only training assistance. 
% %
% We first use the 2D sequence of reconstructed point clouds to generate 2D multi-view features corresponding to all objects to supplement the texture attribute features of objects in 3D point clouds.
% %
% Then we encode the 2D images with CLIP Vision Encoder to obtain the 2D vision tokens corresponding to the 3D objects.
% %
% To transfer the knowledge effectively, we propose a new training schema Visual-Linguistic Semantics Assisted Training (VL-SAT) in 3D Scene Graph Prediction.
% %
% We transfer the knowledge ...

%
% The contribution of our paper can be summarized as (need to be modified):
% %
% 1) We propose a Visual-Linguistic Semantic Assisted Training framework with node and edge-level collaboration and triplet-level regularization to collaboratively boost both oracle model and 3D model.
%  to predict reliable 3D scene graphs
% 1). We use 2D CLIP to fuse with 3D data by mapping method, which complements the color, texture attributes, and semantic features of objects that are difficult to obtain from 3D data through multi-modal fusion, and better extracts the relationship information between 3D objects, which is the first attempt of the pre-trained semantic big model in 3D vision+language task.
%
% 2) We further migrate 2D and language semantics to generate a strong oracle model. To our best knowledge, it is the first time to study the contribution of 2D pretrained model on 3D-VL tasks.
% 2) We propose multiple knowledge migration schemes between different modalities, which can achieve the effect of comprehensive model performance improvement without adding extra computation at the time of inference.
% 3) Experiments show that our method effectively solves the problems of single object relationships and poor tail performance brought by insufficient data volume of 3D Scene Graph.

==> cvpr2023-cross-modal-3dssg/secs/method.tex <==
% !TEX root = ../PaperForReview.tex

\section{Method}
\label{sec:method}

%-------------------------------------------------------------------------
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\linewidth]{picture/arch.pdf}
\caption{
%
\textbf{The proposed Visual-Linguistic Semantics Assisted Training (VL-SAT) for 3D scene graph prediction.}
%
In training, VL-SAT takes 2D and language semantics as extra inputs and helps 3D scene graph prediction with node and edge-level collaboration and triplet-level regularization.
%
In inference, VL-SAT only takes the 3D point cloud to predict reliable 3D scene graphs.
% The network takes in both 3D and 2D inputs: 3D inputs are point clouds of segmented objects and 2D inputs are image patches projected from corresponding 3D objects.
%
% The framework adheres to a teacher-student architecture, in which both teacher and student networks consist of several GNN-based blocks.
%
% The teacher network is further enhanced in three levels: object-level, relation-level and triplet-level.
%
% The student and teacher networks are jointly trained, but only the student network and 3D inputs are used during inference (see the orange arrow).
}
\label{fig:network}
\end{figure*}

We first overview the formulation of 3D semantic scene graph (3DSSG) prediction in point cloud (\cref{sub:problem_formulation}) and then elaborate on a GNN-based network that we experiment on as our 3D prediction model (\cref{sub:baseline}).
%
Since then we highlight how our Visual-Linguistic Semantics Assisted Training (VL-SAT) scheme comprehensively transfers the benefits of an oracle multi-modal prediction model to the 3D prediction model in discriminating challenging relations (\cref{sub:heterogeneous_collaborative_learning}).
%
Finally, we depict the training objective in \cref{sub:training_and_inference}.

\subsection{Problem Formulation}
\label{sub:problem_formulation}

Suppose we have a point cloud $\mP \in \Rbb^{N\times3}$ with $N$ 3D points, and a set of \emph{class-agnostic} instance masks $\cM = \{\mM_1,...,\mM_K\}$ that associate the point cloud $\mP$ with $K$ semantic instances, as indicated by SGPN~\cite{wald2020learning}, we aim at predicting a 3D semantic scene graph as a directed graph $\cG = \{ \cO, \cR \}$.
%
The set of objects $\cO = \{ o_i \}_{i=1}^K$ are all \emph{named} object instances that are specified by instance masks $\cM$. Each edge $r_{ij}$ in $\cR$ depicts the \emph{predicate} in a relation triplet $\langle \emph{subject}, \emph{predicate}, \emph{object} \rangle$, where the head node $o_i$ of this edge is the \emph{subject} and the tail node $o_j$ is the \emph{object}.
%
To be specific, $o_i$ indicates an object label from $N_\text{obj}$ semantic classes.
%
$r_{ij}$ is a predicate label from $N_\text{rel}$ predicate classes.
%
% Note that the number of edges in $\cR$ is $K(K-1)$ since the graph is assumed fully connected.
%


\subsection{3D Prediction Model}
\label{sub:baseline}

As depicted in \cref{fig:network}, our employed 3D prediction model shares a similar network structure as those GNN-based scene graph prediction methods, such as SGFN~\cite{wu2021scenegraphfusion} and $\text{SGG}_\text{point}$~\cite{zhang2021exploiting}, which mainly consists of node encoder, edge encoder, and scene graph reasoning modules.

\vspace{+1mm}
\noindent\textbf{Node Encoder.}
%
Based on one class-agnostic instance mask $\mM_i$ along with the input point cloud $\mP$, we can extract the set of points $\mP_i$ that correspond to one semantic instance. 
%
% Note that the number of points in each instance is different from each other.
%
We employ a simple PointNet~\cite{qi2017pointnet} to extract instance-level features.
%
The node features $\vo_i^\text{3d} \in \Rbb^{D}$ before the GNN-based scene graph reasoning are thus given by these instance-level features.

\vspace{+1mm}
\noindent\textbf{Edge Encoder.}
%
We follow the same practice as in SGFN~\cite{wu2021scenegraphfusion} to encode the edge features for the GNN-based scene graph reasoning.
%
It requires calculating the differences between several attributes between the linked instances. 
%
For each instance, these attributes include the mean $\vmu$ and standard deviation $\vsigma$ of the 3D points, the size $\vb = (b_x, b_y, b_z)$, the volumn $v = b_xb_yb_z$, and the maximum side length $l=\max(b_x, b_y, b_z)$ of the bounding box.
%
Thus the edge features $\vr_{ij}^\text{3d}\in\Rbb^D$ are encoded by projecting the concatenated differences of these attributes between two instances, via multi-layer perceptron (MLP) layers, \ie,
%
\begin{equation}
    \vr_{ij}^\text{3d} = \mathtt{MLP}(\mathtt{cat}(\vmu_i-\vmu_j, \vsigma_i-\vsigma_j,\vb_i-\vb_j,\ln\frac{l_i}{l_j},\ln \frac{v_i}{v_j})),
\end{equation}
where the subscript $i$ indicates the instance $\mP_i$ in the head node, and the $j$ means the instance $\mP_j$ in the tail node.

\vspace{+1mm}
\noindent\textbf{Scene Graph Reasoning.}
%
In our experiment, we apply a similar GNN structure as in SGFN~\cite{wu2021scenegraphfusion}, which utilizes a Feature-wise Attention (FAT) module~\cite{wu2021scenegraphfusion} to pass messages between nodes and edges, and then gets the updated node and edge features.
%
Each GNN module is paired with a multi-head self-attention (MHSA) module, and they are repeated for $T$ times to extract the final node and edge features $\{\tilde{\vo}_i^\text{3d}\}_{i=1,\ldots,K}$ and $\{\tilde{\vr}_{ij}^\text{3d}\}_{i\neq j, i,j=1,\ldots,K}$.
%
% The GNN modules are repeated for $T$ times to extract the final node and edge features $\{\tilde{\vo}_i^\text{3d}\}_{i=1,\ldots,K}$ and $\{\tilde{\vr}_{ij}^\text{3d}\}_{i\neq j, i,j=1,\ldots,K}$.
%
Since then, an object classifier and a predicate classifier are to predict the elements $\{ o_i, r_{ij}, o_j \}$ of each possible relation triplet from the triplet features $\{ \tilde{\vo}_i^\text{3d}, \tilde{\vr}_{ij}^\text{3d}, \tilde{\vo}_j^\text{3d} \}$.
%
These relation triplets finally construct the semantic scene graph $\cG = \{ \cQ, \cR \}$.
%

\vspace{+1mm}
Note that the 3D prediction model does not have to strictly follow the network of SGFN~\cite{wu2021scenegraphfusion}. More recent GNN-based models, such as~$\text{SGG}_\text{point}$~\cite{zhang2021exploiting} can also be applied. In \cref{subsec:ablation}, we show that the proposed VL-SAT scheme can also enhance both baselines with significant gains, validating that our method is generalizable to common 3DSSG prediction models.

\subsection{Visual-Linguistic Semantics Assisted Training}
\label{sub:heterogeneous_collaborative_learning}

In this subsection, we elaborate on how the visual-linguistic semantics assisted training (VL-SAT) scheme can empower the 3D prediction model with sufficient discrimination about long-tailed and ambiguous semantic relation triplets.
%
The key idea is that this discriminative power comes from auxiliarily learning a powerful multi-modal prediction model that receives structural semantics from vision, and language, as well as the 3D geometry from the 3D prediction model.
%
The multi-modal semantics are expected to be heterogeneously aligned with the 3D semantics at the node and edge levels, and the benefits from the oracle model can be efficiently absorbed by the 3D prediction model during the training process.
%
To be specific, we first introduce the applied multi-modal prediction model that has heterogeneous collaboration with the 3D prediction model, and then the auxiliary training strategies that boost the performance of the oracle model and eventually enhance the 3D prediction model.
%
We present the pipeline of VL-SAT in \cref{fig:network}.

\vspace{+1mm}
\noindent\textbf{Multi-modal Prediction Model as the Oracle.}
%
This multi-modal prediction model acts as the oracle to our 3D prediction model. It copies the 3D prediction network in~\cref{sub:baseline} and also learns to predict 3D semantic scene graphs, but its node features are represented by visual features. 
%
These visual features are extracted by a fixed 2D instance encoder, describing RGB image patches that are associated with each point cloud instance $\mP_i$\footnote{Please refer to the supplementary for the details about how to gather associated image patches with each point cloud instance.}. 
%
The edge features of the multi-modal prediction model are encoded in the same way in \cref{sub:baseline}, thus still capturing 3D spatial structures in understanding relations.
%
 
The features of this oracle model heterogeneously collaborate with those in the 3D prediction model at the node and edge levels, which are conducted before and after each GNN layer in the scene graph reasoning module.
%
The former is a node-level collaboration, and the latter is an edge-level collaboration.
%
To be specific, these collaboration operations are implemented by multi-head cross-attention (MHCA) modules~\cite{vaswani2017attention}, where the keys and values are node/edge features from the 3D model, and the queries are their counterparts from the multi-modal model.
%
The node-level collaboration has a distance-aware masking strategy to remove unnecessary attention between instances that are far apart without valid relations.
%
The mask value between two instances $\mP_i$ and $\mP_j$ are learned by
%
\begin{equation}
    D_{ij}^\text{node} = \mathtt{MLP}(\mathtt{cat}(\vmu_i-\vmu_j, \| \vmu_i-\vmu_j\|_2)),
\end{equation}
with respect to the mean coordinates $\vmu_i$ and $\vmu_j$ of the point cloud instances $\mP_i$ and $\mP_j$.
%
The edge-level collaboration does not use a distance-aware masking strategy since the distance between edges is hard to define, thus it is safer to incorporate all edges into attention calculation. 

%
Note that the heterogeneous collaboration is \emph{unidirectional} from the 3D model to the oracle model, while the benefits of the oracle model are passed to the 3D model through the back-propagated gradient flows.
%
It favors that in the inference stage, predicting 3D semantic scene graphs will not need extra data from other modalities.
%


\vspace{+1mm}
\noindent\textbf{Auxiliary Training Strategies.}
%
% Apart from losses for predicting scene graphs, since the oracle multi-modal model would like to perceive scene graphs also from the visual perspective, it is in nature able to enhanced by visual-linguistic knowledge captured by CLIP~\cite{radford2021learning}.
%
Since the oracle multi-modal model would like to perceive scene graphs from both the visual and linguistic perspective, it is natural to enhance the oracle model using visual-linguistic knowledge captured by CLIP~\cite{gao2021clip}.
%
Specifically, we can generate CLIP text embedding $\ve^{\text{text}}_{ij}$ for each groundtruth relation triplet, and regularize the corresponding triplet features $\{\tilde{\vo}^{\text{oracle}}_i, \tilde{\vr}^{\text{oracle}}_{ij}, \tilde{\vo}^{\text{oracle}}_j\}$ at the end of each GNN layer of the scene graph reasoning module.
%
The CLIP text embeddings are offline extracted by the template ``A scene of a/an [subject][predicate] a/an [object]'' for each GT relation 
%
Thus, the regularization becomes to minimize the embedding distances between the text embeddings $\ve_{ij}^\text{text}$ and the fused triplet features $\vt_{ij}^\text{oracle}$, \ie,
%
\begin{equation}
    L_\text{tri-emb} = \sum_{i=1}^K \sum_{j=1,j\neq i}^K \rho(\vt_{ij}^\text{oracle}, \ve_{ij}^\text{text}) \cdot \Ibb_{[\ve_{ij}^\text{text}~\text{is from GT triplet}]} \label{eq:triplet_embedding_loss}
\end{equation}
%
where $\vt_{ij}^\text{oracle} = \mathtt{MLP}(\mathtt{cat}(\tilde{\vo}_i^\text{oracle}, \tilde{\vr}_{ij}^\text{oracle}  ,\tilde{\vo}_j^\text{oracle}))$ is the fused embedding of the concatenated features $\tilde{\vo}_i^\text{oracle}, \tilde{\vr}_{ij}^\text{oracle}$, and  $\tilde{\vo}_j^\text{oracle}$.
%
$\rho(\cdot, \cdot)$ is a distance metric, we can apply $\ell_1$ norm or negative cosine distance.
%
$\Ibb_{[\cdot]}$ is an indicator function that equals to $1$ when the argument is true, and $0$ otherwise.
%
Thus \cref{eq:triplet_embedding_loss} only regularizes the node and edge features whose triplets have ground-truth relations. 

In addition, before being put into the scene graph reasoning modules, the 3D node features $\vo_i^\text{3d}$ from the 3D model and the 2D node features $\vo_i^\text{2d}$ from the oracle model can be aligned. 
%
We apply a same distance measurement as \cref{eq:triplet_embedding_loss},
%
\begin{equation}
    L_\text{node-init} = \sum_{i=1}^K \rho(\vo_i^\text{3d}, \vo_i^\text{2d}).
\end{equation}
%
To enhance the representation ability of the initialized 2D node features, the 2D instance encoder is a fixed CLIP-pretrained vision encoder.
%
Moreover, to enhance the object classifiers of both models, we use the CLIP object embeddings to initialize the weights of the object classifiers both at the 3D prediction model and the oracle multi-modal prediction model, as in~\cite{radford2021learning,liao2022gen}.

\subsection{The Training Objective}
\label{sub:training_and_inference}
% In this subsection, we discuss the processes of network training and inference.
%
% \noindent\textbf{Training Objective.}
%
% \textcolor{blue}{To be revised.}
The training objective of the entire network is defined as:
\begin{multline}
L = \lambda_{\text{obj}}(L_{\text{obj}}^{\text{3d}}+L_{\text{obj}}^{\text{oracle}}) + \lambda_{\text{pred}}(L_{\text{pred}}^{\text{3d}}+L_{\text{pred}}^{\text{oracle}}) + \\ \lambda_{\text{aux}}(L_{\text{tri-emb}}+L_{\text{node-init}})
\label{eq:loss_total}
\end{multline}
%
$L_{\text{obj}}$ indicates object classification loss and is implemented with cross-entropy loss.
%
$L_{\text{obj}}^{\text{3d/oracle}}$ is applied on 3D/oracle object classifier.
%
$L_{\text{pred}}$ indicates predicate classification loss and is formulated as per-class binary cross-entropy loss as in ~\cite{wald2020learning}.
%
$L_{\text{pred}}^{\text{3d/oracle}}$ is applied on 3D/oracle predicate classifier.
%
$\lambda_{\text{node}}$, $\lambda_{\text{edge}}$, $\lambda_{\text{aux}}$ are hyper-parameters to balance each loss in the same scale.

%
% In train stage, the 3D prediction model and oracle multi-modal model are jointly trained.
% %
% During inference time, only the 3D prediction model is utilized with point cloud-only input.

==> cvpr2023-cross-modal-3dssg/secs/rel.tex <==
% !TEX root = ../PaperForReview.tex

\section{Related Work}
\label{sec:related_work}

\noindent\textbf{Scene Graph Prediction in Point Cloud.}
% %
% Scene Graph Generation (SGG) on images has become a popular task ~\cite{zellers2018neural, yang2018graph, xu2017scene, tang2020unbiased, suhail2021energy, woo2018linknet, chen2019knowledge, tang2019learning} in the last few years, which aims to detect objects and relationships between objects from images. 
% %
% However, because of the lack of spatial structure information, SGG on images has some limitations for the understanding of the positional relationship along the depth between objects.
% %
% Recently, Scene Graph Datasets on 3D gets attention. 
% %
% Armeni \etal first present a 3D scene graph dataset, which maps a space into the form of hierarchical structure, \eg building, room, object, camera.
% %
% But it just predicts the relationships derived from detected object instances on images.
% %
% 3DSSG~\cite{wald2020learning} is another Scene Graph dataset on Point Cloud, and it predicts the Scene Graph directly from point clouds and class-agnostic instance segmentation mask.
% %
% SGFN~\cite{wu2021scenegraphfusion} extends the dataset based on 3DSSG, which aims to generate scene graphs incrementally from the local point clouds restructured by RGB-D sequences.
% %
% While textual information is lost on point clouds, predicting a scene graph directly from it will miss some important cues.
% %
% Our methods follow the task in SGPN~\cite{wald2020learning}, which solves the above problem by involving 2D semantics.
Image-based semantic scene graph prediction has been extensively studied~\cite{zellers2018neural,yang2018graph,xu2017scene,tang2020unbiased,suhail2021energy,woo2018linknet,chen2019knowledge,tang2019learning}in recent years, but only a few works try to predict 3D semantic scene graph in the point cloud.
%
% Scene graph prediction by 2D images is a popular research area~\cite{zellers2018neural,yang2018graph,xu2017scene,tang2020unbiased,suhail2021energy,woo2018linknet,chen2019knowledge,tang2019learning} in the past few years, which aims to detect objects and relationships among objects.
% %
% However, previous researches focuses on 2D images, and relationships in 3D scene are less explored.
% However, limited by 2D images, it is difficult to model many relationships in the real 3D world.
% 
% Recently, scene graph prediction from point clouds draws more attention.
%
Armeni~\etal~\cite{armeni20193d} presented the first 3D scene graph dataset, which maps 3D buildings into hierarchical structures.
%
Wald~\etal~\cite{wald2020learning} constructed a point cloud-based semantic scene graph dataset, namely 3DSSG, with a GNN-based baseline model named SGPN. 
%
The follow-up work SGFN~\cite{wu2021scenegraphfusion} predicted 3DSSG incrementally from RGB-D sequences.
%
In recent years, a few methods were proposed to improve the GNN-based baseline.
% 
% \revise{SGG\_point intro.}
% 
\sggpoint~\cite{zhang2021exploiting} used an edge-oriented graph convolution network to exploit multi-dimensional edge features for relation modeling.
%
Zhang~\etal~\cite{zhang2021knowledge} proposed a graph auto-encoder network to automatically learn a group of embeddings for each class in advance, and then perform the 3DSSG prediction to recognize credible relation triplets from pre-learned knowledge.
% 
% However, these methods do 2D projections, where external knowledge from rich pretraining data can be introduced.

\vspace{+1mm}
\noindent\textbf{3D Scene Understanding with 2D Semantics.}
%
% In the past few years, multi-modality methods have caught considerable attention.
%
% To increase the attribute information of objects in Point Clouds, various tasks utilize 2D images to complement 3D.
%
A list of methods have employed 2D semantics to help 3D instance-level tasks, such as 3D object detection, segmentation, visual grounding and dense captioning~\cite{qi2018frustum,qi2020imvotenet,bai2022transfusion,sindagi2019mvx,vora2020pointpainting,yin2021multimodal,zhi2021place}. They can be coarsely divided into two categories, \ie, concatenating image features with each 3D point~\cite{chen2020scanrefer, zhao20213dvg, cai20223djcg, bai2022transfusion,vora2020pointpainting,yin2021multimodal,qi2020imvotenet}, and projecting object detection results into 3D space~\cite{pang2020clocs, yang2021sat, yuan2022x, qi2018frustum, xu2018pointfusion, lahoud20172d}.
%
Most methods require 2D semantics both in the training and inference stages.
%
Recently, SAT~\cite{yang2021sat} and $\cX$-Trans2Cap~\cite{yuan2022x} explore using 2D semantics only in training to assist 3D visual grounding and dense captioning. Both of them can learn enhanced models that only use 3D inputs in inference.
%
But these methods are restrained to instance-level tasks and the networks have to be carefully designed.
%
% There are mainly two types of approaches that align 3D and 2D semantics.
% % todo
% One is to project 3D detected or Ground-Truth boxes to 2D frames, like ~\cite{yang2021sat}, which prefers to focus on object-level tasks.
% %
% This method has a better representation because of the high accuracy of projection results.
% %
% The other is just the opposite, \ie project 2D pixel-level feature to 3D points, \eg 3DVG~\cite{zhao20213dvg} and 3DJCG~\cite{cai20223djcg}.
% %
% This method needs to save features on a larger receptive field, which is space-consuming.
% %
% Since 3D Scene Graph Prediction on 3DSSG obtains instance segmentation during training, we just use the first type method to generate object-level features.
% %
% Previous studies have added 2D as an additional input to 3D Perception tasks, using  various fusion techniques.
% %
% Yang \etal \cite{yang2021sat} propose that extra 2D inputs potentially limit the application scenarios since the 2D information either does not exist in inference.
%
We follow similar ideas as~\cite{yang2021sat,yuan2022x} and use 2D semantics only in training, but we would like to enhance the 3DSSG prediction that requires structural understanding rather than instance-level perception.

\vspace{+1mm}
\noindent\textbf{Knowledge-inserted Methods in Scene Graph Prediction.}
%
% According to the knowledge source, we can divide the previous studies into two directions.
% %
% The first is to use the prior knowledge from the training dataset.
%
Zellers~\etal~\cite{zellers2018neural} and Chen~\etal~\cite{chen2019knowledge} indicated that the statistical co-occurrences between object pairs and relationships are useful for relation prediction.
%
%  also use the same statistical priors and incorporates them into graph propagation networks to solve the long-tail problem in Scene Graph Generation.
%
Besides, \cite{sharifzadeh2021classification, zhang2021knowledge} generated class-level prototypical representations from all previous perceptual outputs as the prior knowledge.
%
These methods explicitly encoded the data priors into the model.
%
% The other is to utilize the knowledge from the extra database.
%
% To dismiss the huge variations in the visual appearances between the same predicate, which has a different object/subject, 
%
\cite{li2017vip, lu2016visual, liao2019natural, abdelkarim2021exploring} attempted to combine language priors with scene graph prediction.
%
% Furthermore, commonsense knowledge is also utilized to assist the task.
%
Zareian~\etal~\cite{zareian2020bridging} proposed a Graph Bridging Network to propagate messages between scene graphs and knowledge graphs.
%
% They encode the commonsense using language models, which ignores the commonsense hidden in vision.
%
Our VL-SAT scheme uses CLIP to encode the linguistic semantics, which is thus better aligned with 2D semantics, and even the required 3D structural semantics during the training stage.
%
